GOALS-JWST: Tracing AGN Feedback on the Star-Forming ISM in NGC 7469

We present James Webb Space Telescope (JWST) Mid-InfraRed Instrument (MIRI) integral-field spectroscopy of the nearby merging, luminous infrared galaxy, NGC 7469. This galaxy hosts a Seyfert type-1.5 nucleus, a highly ionized outflow, and a bright, circumnuclear star-forming ring, making it an ideal target to study AGN feedback in the local Universe. We take advantage of the high spatial/spectral resolution of JWST/MIRI to isolate the star-forming regions surrounding the central active nucleus and study the properties of the dust and warm molecular gas on ~100 pc scales. The starburst ring exhibits prominent Polycyclic Aromatic Hydrocarbon (PAH) emission, with grain sizes and ionization states varying by only ~30%, and a total star formation rate of $\rm 10 - 30 \ M_\odot$/yr derived from fine structure and recombination emission lines. Using pure rotational lines of H2, we detect 1.2$\times$10$^{7} \rm \ M_\odot$ of warm molecular gas at a temperature higher than 200 K in the ring. All PAH bands get significantly weaker towards the central source, where larger and possibly more ionized grains dominate the emission. However, the bulk of the dust and molecular gas in the ring appears unaffected by the ionizing radiation or the outflowing wind from the AGN. These observations highlight the power of JWST to probe the inner regions of dusty, rapidly evolving galaxies for signatures of feedback and inform models that seek to explain the co-evolution of supermassive black holes and their hosts.

==> tab1_PAH_Ne.tex <==
\begin{deluxetable*}{@{\extracolsep{4pt}}lccccccc}%{cccccccc}
\tabletypesize{\footnotesize}
\tablewidth{0pt}
 \tablecaption{PAH Band and Emission Line Fluxes }\label{tab:flux}

 \tablehead{
 \colhead{Regions} & \colhead{R.A.} & \colhead{Dec.} & \colhead{PAH 6.2\um} & \colhead{PAH 7.7\um} & \colhead{PAH 11.3\um} & \colhead{[NeII] 12.81\um} & \colhead{[NeIII] 15.56\um} \\
 \cline{4-6} \cline{7-8}
 \colhead{} & \colhead{(ICRS)} & \colhead{(ICRS)} & \multicolumn{3}{c}{($\times$10$^{-16}$ W/m$^{2}$)} & \multicolumn{2}{c}{($\times$10$^{-17}$ W/m$^{2}$)}\\ [-0.4cm]
%  \colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} & \colhead{(6)} & \colhead{(7)}  & \colhead{(8)}\\
 }
 \startdata 
R1  &  23:03:15.5147 & +8:52:25.111 & 5.31 $\pm$ 0.19 & 20.61 $\pm$ 1.04 & 4.80 $\pm$ 0.25 & 12.07 $\pm$ 0.16 & 1.14 $\pm$ 0.03 \\
R2  &  23:03:15.5791 & +8:52:24.734 & 4.72 $\pm$ 0.10 & 15.29 $\pm$ 0.61 & 4.34 $\pm$ 0.16 & 17.16 $\pm$ 0.13 & 1.28 $\pm$ 0.02 \\
R3  &  23:03:15.6279 & +8:52:25.076 & 3.64 $\pm$ 0.11 & 12.78 $\pm$ 0.74 & 3.24 $\pm$ 0.16 &  7.41 $\pm$ 0.08 & 1.44 $\pm$ 0.02 \\
R4  &  23:03:15.7021 & +8:52:25.267 & 3.65 $\pm$ 0.18 & 11.58 $\pm$ 0.86 & 3.28 $\pm$ 0.30 &  8.06 $\pm$ 0.06 & 1.03 $\pm$ 0.02 \\
R5  &  23:03:15.6789 & +8:52:25.999 & 4.04 $\pm$ 0.09 & 16.12 $\pm$ 0.58 & 3.83 $\pm$ 0.09 &  8.17 $\pm$ 0.07 & 2.54 $\pm$ 0.03 \\
R6  &  23:03:15.7192 & +8:52:26.531 & 3.36 $\pm$ 0.12 & 13.24 $\pm$ 0.64 & 3.51 $\pm$ 0.20 &  6.62 $\pm$ 0.05 & 0.95 $\pm$ 0.02 \\
R7  &  23:03:15.6853 & +8:52:27.197 & 3.71 $\pm$ 0.07 & 12.63 $\pm$ 0.40 & 4.02 $\pm$ 0.08 & 11.24 $\pm$ 0.07 & 1.14 $\pm$ 0.02 \\
R8  &  23:03:15.6422 & +8:52:27.714 & 3.29 $\pm$ 0.10 & 10.72 $\pm$ 0.52 & 2.69 $\pm$ 0.12 &  5.95 $\pm$ 0.04 & 0.68 $\pm$ 0.01 \\
R9  &  23:03:15.5919 & +8:52:27.380 & 4.35 $\pm$ 0.08 & 15.98 $\pm$ 0.53 & 3.61 $\pm$ 0.10 &  8.67 $\pm$ 0.07 & 1.30 $\pm$ 0.02 \\
R10 &  23:03:15.5482 & +8:52:26.884 & 3.54 $\pm$ 0.10 & 13.75 $\pm$ 0.76 & 3.24 $\pm$ 0.15 &  8.27 $\pm$ 0.07 & 1.29 $\pm$ 0.02 \\
R11 &  23:03:15.5096 & +8:52:26.217 & 3.74 $\pm$ 0.10 & 13.68 $\pm$ 0.57 & 3.62 $\pm$ 0.18 &  8.92 $\pm$ 0.06 & 1.02 $\pm$ 0.01 \\
R1a &  23:03:15.5366 & +8:52:25.419 & 6.37 $\pm$ 0.27 & 26.14 $\pm$ 1.58 & 6.77 $\pm$ 0.38 & 13.43 $\pm$ 0.18 & 2.55 $\pm$ 0.05 \\
R2a &  23:03:15.5881 & +8:52:25.210 & 6.18 $\pm$ 0.16 & 23.24 $\pm$ 1.02 & 5.79 $\pm$ 0.21 & 15.72 $\pm$ 0.13 & 2.05 $\pm$ 0.03 \\
R7a &  23:03:15.6621 & +8:52:26.797 & 3.68 $\pm$ 0.08 & 14.57 $\pm$ 0.53 & 3.88 $\pm$ 0.07 & 10.06 $\pm$ 0.08 & 2.53 $\pm$ 0.03 \\
R10a &  23:03:15.5728 & +8:52:26.578 & 2.22 $\pm$ 0.07 & 8.87 $\pm$ 0.31 & 2.27 $\pm$ 0.02 & 6.38 $\pm$ 0.08 & 2.83 $\pm$ 0.06 \\
R2b &  23:03:15.6011 & +8:52:25.619 & 6.16 $\pm$ 0.40 & 25.75 $\pm$ 2.36 & 6.16 $\pm$ 0.18 & 13.19 $\pm$ 0.18 & 7.50 $\pm$ 0.12 \\
R7b &  23:03:15.6401 & +8:52:26.555 & 2.24 $\pm$ 0.17 &  9.60 $\pm$ 0.76 & 1.48 $\pm$ 0.05 &  5.10 $\pm$ 0.08 & 5.48 $\pm$ 0.08 \\
Nucleus & 23:03:15.6155 & +8:52:26.180 & 1.59 $\pm$ 0.26 & 5.24 $\pm$ 0.31 & 0.87 $\pm$ 0.14 & 7.63 $\pm$ 0.28 & 12.19 $\pm$ 0.27
 \enddata

 \vspace{-0.5cm}
 %\tablecomments{}
\end{deluxetable*}

==> tab2_H2.tex <==
\begin{deluxetable*}{lccccccccccccc}
\tabletypesize{\footnotesize}
\tablewidth{0pt}
 \tablecaption{\molH\ Line Fluxes}\label{tab:h2_flux}

 \tablehead{
 \colhead{Regions} & \colhead{S(1)} & \colhead{S(2)} & \colhead{S(3)} & \colhead{S(4)} & \colhead{S(5)} & \colhead{S(6)} & \colhead{S(7)} \\ [-0.2cm] 
 \colhead{} & \colhead{17.04\um} & \colhead{12.28\um} & \colhead{9.67\um} & \colhead{8.03\um} & \colhead{6.91\um} & \colhead{6.11\um} & \colhead{5.51\um} \\ 
 [-0.4cm] 
 }
%\vspace{-10pt}
 \startdata 
R1  & 4.70 $\pm$ 0.33 & 2.55 $\pm$ 0.08 & 3.95  $\pm$ 0.17 & 1.65 $\pm$ 0.13 & 3.08  $\pm$ 0.10 & 0.50 $\pm$ 0.07 & 1.34 $\pm$ 0.05 \\
R2  & 4.63 $\pm$ 0.15 & 2.38 $\pm$ 0.09 & 3.43  $\pm$ 0.10 & 1.35 $\pm$ 0.09 & 2.55  $\pm$ 0.08 & 0.36 $\pm$ 0.10 & 0.98 $\pm$ 0.07 \\
R3  & 1.83 $\pm$ 0.53 & 1.80 $\pm$ 0.07 & 2.48  $\pm$ 0.11 & 0.97 $\pm$ 0.07 & 1.71  $\pm$ 0.08 & 0.33 $\pm$ 0.05 & 0.59 $\pm$ 0.06 \\
R4  & 4.29 $\pm$ 0.22 & 2.17 $\pm$ 0.07 & 3.20  $\pm$ 0.09 & 1.04 $\pm$ 0.06 & 1.98  $\pm$ 0.07 & 0.40 $\pm$ 0.03 & 0.82 $\pm$ 0.06 \\
R5  & 4.31 $\pm$ 0.30 & 2.52 $\pm$ 0.12 & 3.95  $\pm$ 0.15 & 1.71 $\pm$ 0.09 & 3.00  $\pm$ 0.12 & 0.55 $\pm$ 0.10 & 1.27 $\pm$ 0.08 \\
R6  & 4.80 $\pm$ 0.12 & 2.41 $\pm$ 0.09 & 3.28  $\pm$ 0.09 & 1.26 $\pm$ 0.06 & 2.24  $\pm$ 0.12 & 0.36 $\pm$ 0.06 & 0.88 $\pm$ 0.15 \\
R7  & 4.08 $\pm$ 0.20 & 2.25 $\pm$ 0.06 & 3.64  $\pm$ 0.08 & 1.36 $\pm$ 0.06 & 2.46  $\pm$ 0.09 & 0.45 $\pm$ 0.05 & 1.24 $\pm$ 0.13 \\
R8  & 3.76 $\pm$ 0.07 & 1.91 $\pm$ 0.06 & 3.25  $\pm$ 0.10 & 1.19 $\pm$ 0.06 & 2.09  $\pm$ 0.07 & 0.37 $\pm$ 0.10 & 0.91 $\pm$ 0.06 \\
R9  & 1.79 $\pm$ 0.58 & 2.20 $\pm$ 0.06 & 3.36  $\pm$ 0.19 & 1.49 $\pm$ 0.07 & 2.48  $\pm$ 0.09 & 0.43 $\pm$ 0.05 & 1.12 $\pm$ 0.07 \\
R10 & 3.31 $\pm$ 0.29 & 1.78 $\pm$ 0.07 & 2.73  $\pm$ 0.12 & 1.09 $\pm$ 0.06 & 1.86  $\pm$ 0.07 & 0.28 $\pm$ 0.05 & 0.88 $\pm$ 0.08 \\
R11 & 3.31 $\pm$ 0.13 & 1.69 $\pm$ 0.07 & 2.48  $\pm$ 0.14 & 0.96 $\pm$ 0.06 & 1.62  $\pm$ 0.08 & 0.31 $\pm$ 0.06 & 0.61 $\pm$ 0.07 \\
R1a & 9.74 $\pm$ 0.36 & 4.82 $\pm$ 0.14 & 7.81  $\pm$ 0.19 & 3.28 $\pm$ 0.14 & 5.36  $\pm$ 0.13 & 1.05 $\pm$ 0.12 & 2.55 $\pm$ 0.14 \\
R2a & 6.19 $\pm$ 0.24 & 3.14 $\pm$ 0.12 & 5.16  $\pm$ 0.20 & 2.34 $\pm$ 0.10 & 3.75  $\pm$ 0.13 & 0.52 $\pm$ 0.13 & 1.75 $\pm$ 0.11 \\
R7a & 4.44 $\pm$ 0.19 & 2.88 $\pm$ 0.08 & 4.86  $\pm$ 0.13 & 2.07 $\pm$ 0.09 & 3.83  $\pm$ 0.09 & 0.63 $\pm$ 0.05 & 1.73 $\pm$ 0.11 \\
R10a & 3.56 $\pm$ 0.48 & 3.29 $\pm$ 0.20 & 6.94 $\pm$ 0.36 & 3.24 $\pm$ 0.22 & 6.00 $\pm$ 0.22 & 1.16 $\pm$ 0.12 & 2.97 $\pm$ 0.10 \\
R2b & 4.15 $\pm$ 0.76 & 4.76 $\pm$ 0.55 & 10.11 $\pm$ 0.53 & 6.36 $\pm$ 0.46 & 12.44 $\pm$ 0.37 & 2.53 $\pm$ 0.21 & 6.80 $\pm$ 0.51 \\
R7b & 3.38 $\pm$ 0.71 & 2.20 $\pm$ 0.30 & 3.83  $\pm$ 0.25 & 2.61 $\pm$ 0.33 & 5.66  $\pm$ 0.07 & 1.14 $\pm$ 0.06 & 3.07 $\pm$ 0.57 \\
Nucleus & 3.79 $\pm$ 1.45 & 2.77 $\pm$ 1.29 & 6.01 $\pm$ 0.59 & 4.70 $\pm$ 0.52 & 10.89  $\pm$ 0.21 & 2.24 $\pm$ 0.14 & 6.22 $\pm$ 1.92 \\
 \enddata
 \tablecomments{All \molH\ pure rotational line fluxes are in unit of 10$^{-18}$ W/m$^{2}$.}
\end{deluxetable*}
